InternVideo2: Scaling Foundation Models for Multimodal Video Understanding

We introduce InternVideo2, a new family of video foundation models (ViFM) that achieve the state-of-the-art results in video recognition, video-text tasks, and video-centric dialogue. Our core design is a progressive training approach that unifies the masked video modeling, crossmodal contrastive learning, and next token prediction, scaling up the video encoder size to 6B parameters. At the data level, we prioritize spatiotemporal consistency by semantically segmenting videos and generating video-audio-speech captions. This improves the alignment between video and text. Through extensive experiments, we validate our designs and demonstrate superior performance on over 60 video and audio tasks. Notably, our model outperforms others on various video-related dialogue and long video understanding benchmarks, highlighting its ability to reason and comprehend longer contexts. Code and models are available at https://github.com/OpenGVLab/InternVideo/tree/main/InternVideo2/.

==> content/data.tex <==
\begin{table*}[t]
% \scriptsize
    \caption{Statistics of pretraining corpus in {\modelname}. }
\small
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l l l l l c} 
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Domain} & \multirow{2}{*}{\#Samples} & \multicolumn{3}{c}{Annotation}  \\
    & & & Mode & Type & \#Avg Tokens\\
    \midrule
    WebVid & Open & 10M & Fusion & Video & -\\
    \dataname~ (ours) & Open & 10M & Generated & Video & 23.4\\
    \dataname2~ (ours) & Open & 40M & Generated & AVS & -\\
    \midrule
    CC12M & Open & 13M & Fusion & Image & -\\
    CC3M & Open & 3M & Fusion & Image & -\\
    SBU & Open & 12M & Fusion & Image & -\\
    Laion-POP & Open & 0.6M & Fusion & Image & - \\
    \bottomrule
    \end{tabular}
% }
    \label{tab:datasets}
\end{table*}

==> content/tables/InternVideo_pretraining_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\caption{Summary of datasets used in \modelname{} pretraining process.}
\resizebox{0.82\textwidth}{!}
{
\begin{tabular}{cllll}
\toprule
\multicolumn{2}{c}{Pretraining   Dataset}                         & Domain            & \# of clips & Annotation            \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{K-mash}}        & K710         & Youtube Video     & 658k        & Action Label          \\
\multicolumn{1}{c|}{}                              & SthSthV2     & Shot from scripts & 169k        & Action Label          \\
\multicolumn{1}{c|}{}                              & HACS         & Youtube Video     & 106k        & Action Label          \\
\multicolumn{1}{c|}{}                              & Anet         & Youtube Video     & 15k         & Action Label          \\
\multicolumn{1}{c|}{}                              & MiT          & Web Video         & 207k        & Action Label          \\
\multicolumn{1}{c|}{}                              & Self-collect & Youtube Video     & 844k        & Caption, Action Label \\ \midrule
\multicolumn{1}{c|}{\multirow{11}{*}{Vision-Text}} & LAION-2B     & Web Image         & 158M        & Alt-text              \\
\multicolumn{1}{c|}{}                              & LAION-COCO    & Web Image         & 117M   & Generated Caption     \\
\multicolumn{1}{c|}{}                              & LAION-POP    & Web Image         & 611k        & Generated Caption     \\
\multicolumn{1}{c|}{}                              & All-Seeing   & HQ Image          & 11M         & Generated Caption     \\
\multicolumn{1}{c|}{}                              & CC12M        & Web Image         & 13M         & Alt-text              \\
\multicolumn{1}{c|}{}                              & SBU          & Flickr            & 1.2M        & Handcrafted  Caption  \\
\multicolumn{1}{c|}{}                              & VG           & Flickr            & 108k        & Handcrafted Caption   \\
\hline
\multicolumn{1}{c|}{\multirow{6}{*}{Instruction Data}}                              & LLaVA     & Web Image         & 157k        & Conversation, Caption              \\
\multicolumn{1}{c|}{}                              & MiniGPT-4    & Web Image         & 3k        & Caption               \\
\multicolumn{1}{c|}{}                              & VideoChat    & Web Video         & 21k        & Conversation, Caption               \\
\multicolumn{1}{c|}{}                              & VideoChatGPT    & Web Video         & 13k        & Conversation               \\
\multicolumn{1}{c|}{}                              & VideoChat2-IT    & Image & Video     & 1.9M         & Conversation, Caption    \\
\bottomrule
\end{tabular}
}
\label{tab:pretrain_data}
\end{table}

==> content/tables/architecture.tex <==
\begin{table}[tp]
    \centering
    % \setlength\tabcolsep{8.0pt}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{c|c|c}
        \textbf{Stage} & \textbf{ViT-6B} & \textbf{Output Size} \\
        \Xhline{1.0pt}
        Video & sparse sampling & \violet{3}$\times$\darkGreen{8}$\times$\myblue{224}$\times$\myblue{224} \\
        \hline
        Patch & \darkGreen{1}$\times$\myblue{14}$\times$\myblue{14}, \violet{3200} & \multirow{2}{*}{\violet{3200}$\times$\darkGreen{8}$\times$\orange{256}} \\
        Embedding & stride \darkGreen{1}$\times$\myblue{14}$\times$\myblue{14} & ~ \\
        \hline
        Position & learnable, 3D sine-cosine initialization & \multirow{2}{*}{\violet{3200}$\times$\orange{2048}} \\
        Embedding & \violet{3200}$\times$\orange{2048} & ~ \\
        \hline
        Mask & semantic mask w/ \textit{mask ratio} $=$ $\rho$ & \violet{3200}$\times$\orange{2048$\cdot$(1-$\rho$)} \\
        \hline
        Encoder & $\left[\begin{array}{c}\text{MHSA(\violet{3200})}\\\text{MLP(\violet{12800})}\end{array}\right]$$\times$48 $+$ AttnPool(\violet{768}) & 
        \makecell{\violet{3200}$\times$\orange{2048$\cdot$(1-$\rho$)}
        \\\violet{768}$\times$\orange{1}} \\
        \hline
        Projection & 
        $\left[\begin{array}{c}\text{LN(\violet{3200})}\\\text{MLP(\violet{3200})}\end{array}\right]$$\times$$K_{CLIP}$,
        $\left[\begin{array}{c}\text{LN(\violet{3200})}\\\text{MLP(\violet{1408})}
        \end{array}\right]$$\times$$K_{MAE}$,
        $\left[\begin{array}{c}\text{LN(\violet{3200})}\\\text{MLP(\violet{768})}
        \end{array}\right]$$\times1$ & 
        \makecell{$K$$\times$\violet{3200}$\times$\orange{2048$\cdot$(1-$\rho$)}
        \\$K$$\times$\violet{1408}$\times$\orange{2048$\cdot$(1-$\rho$)}
        \\$K$$\times$\violet{768}$\times$\orange{1}} \\
        % \hline
        % \multirow{2}{*}{Target} & unmasked token & \multirow{2}{*}{$K$$\times$\violet{512}$\times$\darkGreen{8}$\times$[196$\cdot$(1-$\rho$)]} \\
        % ~ & alignment & ~ \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \caption{\textbf{Architecture of vision encoder.}
    We take ViT-6B as an example and omit the class token for a simple presentation.
    ``MHSA'', ``MLP'', ``AttnPool'', and ``LN'' refer to spatiotemporal multi-head self-attention, multi-layer perception, attention pooling~\citep{coca} and root mean square layer normalization~\citep{zhang2019root}.
    $K_{CLIP}$ and $K_{MAE}$ means the layer number for unmasked token alignment with multimodal and motion-aware teachers.
    We mark the \violet{channel number}, \darkGreen{frame number}, \myblue{spatial size}, and \orange{token number} by different colors.
    The projection layers are dropped after Stage1 training.
    }
    \label{tab:model_architecture}
    % \vspace{-0.3cm}
\end{table}

==> content/tables/s2_table1.tex <==
\begin{table*}[t]
\scriptsize
% \small
    \centering
    \caption{Data Source Summary}
    \vspace{-0.3cm}
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{r r r r r r r r r r} 
    \toprule
    Dataset & Domain  & Region & \#Samples & Annotation  \\\hline\hline
    % Bilibili & General & China & 173,854 & None \\
    % Douyin & Short Videos & China & 2,439,185 & None \\
    - & Short Videos & China & 2,613,039 & None \\
    IMDB & Movie & Multi & 319,054 & None \\
    Vimeo~\cite{wang2023lavie} & General & Multi & 10,265,705 & Video Caption \\
    YT-Temporal-180M~\cite{zellers2021merlot} & General & Multi & 10,000,000 & ASR \\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:internvid2_datasets_source}
\end{table*}
